IRFL: Image Recognition of Figurative Language

Figures of speech such as metaphors, similes, and idioms are integral parts of human communication. They are ubiquitous in many forms of discourse, allowing people to convey complex, abstract ideas and evoke emotion. As figurative forms are often conveyed through multiple modalities (e.g., both text and images), understanding multimodal figurative language is an important AI challenge, weaving together profound vision, language, commonsense and cultural knowledge. In this work, we develop the Image Recognition of Figurative Language (IRFL) dataset. We leverage human annotation and an automatic pipeline we created to generate a multimodal dataset, and introduce two novel tasks as a benchmark for multimodal figurative language understanding. We experimented with state-of-the-art vision and language models and found that the best (22%) performed substantially worse than humans (97%). We release our dataset, benchmark, and code, in hopes of driving the development of models that can better understand figurative language.

==> sections/08_ethics_statment.tex <==
Idiomatic expressions can sometimes be used as slang for cursing or passing inappropriate messages. We've ensured every query and idiom passes through automatic and manual verification, preventing inappropriate content from infiltrating our dataset. This approach is also applied to the selection of images, considering that idiom definitions can be abstract and appear in varied contexts. We've excluded any visuals we found inappropriate to minimize the potential harm that could come from offensive or inappropriate material. As we do not own or distribute the images used, we will provide their links and acknowledgment to the website they originated from.
% https://www.acm.org/code-of-ethics
% The above follows the 1.2. Avoid harm - "Idiomatic expressions can sometimes be used as slang for cursing or passing inappropriate messages. We've ensured every query and idiom passes through automatic and manual verification, preventing inappropriate content from infiltrating our dataset. This approach is also applied to the selection of images, considering that idiom definitions can be abstract and appear in varied contexts. We've excluded any visuals we found inappropriate to minimize the potential harm that could come from offensive or inappropriate material."
% 1.5 Respect the work required to produce new ideas, inventions, creative works, and computing artifacts. - "As we do not own or distribute the images used, we will provide their links and acknowledgment to the website they originated from."


==> sections/100B_dataset_supplementary_materials.tex <==
\begin{enumerate}
  \item After the review process is complete, dataset documentation, metadata, and download instructions will be released.
  \item Intended uses: We hope researchers will use our benchmarks to evaluate Vision and Language models. We also hope that our pipeline and dataset will inspire future work on creating extensive multimodal datasets of other figures of speech.
  \item Author statement: We bear all responsibility in case of violation of rights in using our benchmark. 
  \item Licenses: Dataset is licensed under CC-BY 4.0 license \url{https://creativecommons.org/licenses/by/4.0/legalcode}.
\end{enumerate}


==> sections/100C_instructions.tex <==

\newpage
\subsection{Instructions}
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-1.jpg}
    \caption{Page 1 out of 8}
    \label{fig:instructions_first_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-2.jpg}
    \caption{Page 2 out of 8}
    \label{fig:instructions_second_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-3.jpg}
    \caption{Page 3 out of 8}
    \label{fig:instructions_three_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-4.jpg}
    \caption{Page 4 out of 8}
    \label{fig:instructions_four_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-5.jpg}
    \caption{Page 5 out of 8}
    \label{fig:instructions_five_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-6.jpg}
    \caption{Page 6 out of 8}
    \label{fig:instructions_six_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-7.jpg}
    \caption{Page 7 out of 8}
    \label{fig:instructions_seven_page}
\end{figure}
\end{center}
\newpage
\begin{center}
\begin{figure}
    \centering
    \includegraphics[width=12cm,height=30cm,keepaspectratio]{instructions/instructions_for_paper-8.jpg}
    \caption{Page 8 out of 8}
    \label{fig:instructions_eight_page}
\end{figure}
\end{center}
\newpage

==> sections/100E_annotation_task_discussion.tex <==
The nature of the image annotation task is very subjective, and often the relation worker A sees between an idiom and an image differs from the relation worker B sees. The connection a worker sees between an image and an idiom can vary based on his understanding of the image scene and his interpretation of that scene. For example, Figure~\ref{fig:tiget_by_the_tail} shows a "Literal" image of a person holding a tiger by the tail in a non-dangerous or difficult situation in which one should not remain. The person is smiling as it seems like he is playing with a very young tiger (small in size). The majority of workers agreed with this explanation, except one who disagreed and chose the "Figurative Literal" category. This worker's interpretation arose from her viewpoint as a mother, and she said, "as a mother, I would still say that it's dangerous and the person is being foolish".\\
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.40\textwidth,height=12cm,keepaspectratio]{figures/Figure_104_have_a_tiger_by_the_tail.JPG}
    \caption{A candidate image from the training platform.}
    \label{fig:tiget_by_the_tail}
\end{figure}
\newline\noindent Another example of different interpretations is the image seen in Figure~\ref{fig:cowboy_bunny}, which shows an image of a cowboy bunny drawing with the idiom - "quick on the draw". The annotations of this image were very diverse as $5$ workers chose $4$ different categories. Two workers chose "Figurative" as they saw a connection to the idiom definitions. One worker chose "Figurative Literal" as he saw a connection to the idiom definitions and a literal connection to the idiom. Another worker chose "Literal" because he did not find the image to be "Figurative" and saw the idiom literally as illustrating the image. The last worker selected "None" as he did not find a clear literal connection and didn't see the image as "Figurative" as it lacked an indication that the bunny was "quick to act" or "characterized by rapid response".
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.40\textwidth,height=12cm,keepaspectratio]{figures/Figure_103_cowboy_bunny.JPG}
    \caption{A figurative candidate of the idiom "quick on the draw".}
    \label{fig:cowboy_bunny}
\end{figure}



==> sections/Old_05B_expiremnets_details.tex <==
We introduce two novel tasks of multimodal figurative language detection and retrieval to evaluate humans and state-of-the-art models' ability to understand figurative language (\S\ref{sec:understanding_task}).

The {\bf  Multimodal Figurative Language Detection Task} evaluates VL-PTMs’ ability to understand the relation between an image and a figurative phrase. The task is to choose the image that best visualizes the figurative phrase out of X candidates. Figure~\ref{fig:first-task-idiom-figurative} shows an example of the task for an idiom, a metaphor, and a simile.

The {\bf Multimodal Figurative Retrieval Task} examines VL-PTMs' preference for figurative images. The task is to rank the figurative and partially literal images using the model-matching score and calculate the precision at $k$, where $k$ is the number of figurative images. Figure~\ref{fig:second-task-idiom-figurative-vs-caption} shows an example of the task for the idiom ``ruffle someone's feathers''.

We show that IRFL tasks are easy for humans (97\% accuracy) and challenging for models (<22\%). Additionally, we provide a detailed analysis per figure of speech, experiments with idioms and their definitions as input, and with different candidate types. We find that models fail the IRFL task due to their preference for partially literal images over figurative images and introduce a retrieval task to tackle this problem (\S\ref{sec:ranking Task Analysis}). In addition, we examine the ability of generative models such as Dall-E and Stable Diffusion to generate figurative images for idioms (\S\ref{sec:genearive_models_analysis}). We find that they are unable to generate figurative images given idiomatic phrases. However, given the definitions of an idiom, generative models can generate figurative images.






==> tables/backup.tex <==
\begin{table}[h]
\centering
\scalebox{0.6}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
Categories   & \multicolumn{3}{c}{Figurative} & Figurative+Literal & Caption & Partial Objects\\ \midrule
Candidates  &  2 & 4 & 6          & 4                & 4       & 4 \\ \midrule
CLIP-VIT-L/14   &  \textbf{52} & \textbf{42} & \textbf{34}  & \textbf{87} & \textbf{98}    & \textbf{88} \\
CLIP-VIT-B/32   &  61 & 39 & 30          & 80                & 93       & \textbf{88} \\
CLIP-RN50       &  59 & 36 & 34      & 79                & 94       & 86 \\

CLIP-RN50x64/14 &  61 & 41 & 34          & 84                & 95       & 84\\
LiT             &  47 & 28 & 13         & 33                & 32       & 26 \\ \bottomrule

\end{tabular}}
\caption{Zero-shot models performance on the IRFL dataset. Numbers are the percentage of instances annotated correctly. Bold numbers indicate the best model performances. There are three configurations for the Figurative Category with 2, 4 and 6 candidates. Adding or decreasing the number of candidates for other categories affected the results only slightly for 2 and 6 candidates.}
\label{tab:idiom-single-choice-results}
\end{table}
\ron{Remove human performance from this tab and put it only on mix}
\ron{Create very diverse task and start with it}
\ron{Fine-grained analysis - distractors affect}
\ron{to better understand the behavior of these models on the dataset, we examine other categories}






==> tables/old_generative_models_baseline_vs_irfl.tex <==
\begin{table}[h!]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}lccccc@{}}
\toprule
Categories         & Dall E & \begin{tabular}[c]{@{}l@{}}Stable \\ Diffusion\end{tabular} & IRFL & \\ \midrule
Figurative         & 31\%                         & 8\%              &  33\%                 \\
Figurative+Literal & 7\%                          & 2\%              &  12\%           \\
Literal            & 9\%                          & 6\%              &  13\%        \\
Partial Literal    & 15\%                         & 16\%             &  10\%          \\
None               & 38\%                         & 68\%             &  32\%       \\ \midrule
Number             & 165                          & 171               & 181  \\ \bottomrule 
\end{tabular}} 
\caption{The table describes the percentage of images generated by idioms and their definitions that fit the category. }
\label{tab:generative_models_baseline_vs_irfl}
\end{table}


==> tables/partial-backup.tex <==
\begin{table}[h]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
Categories   & \multicolumn{2}{c}{Figurative}\\ \midrule
Candidates  &                      2                           &                      4 \\ \midrule
CLIP-VIT-L/14   &  \begin{tabular}[c]{@{}l@{}}8\% 18\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}1\% 7\%\end{tabular} \\
CLIP-VIT-B/32   &  \begin{tabular}[c]{@{}l@{}}6\% 20\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}0\% 7\%\end{tabular} \\
CLIP-RN50       &  \begin{tabular}[c]{@{}l@{}}6\% 18\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}1\% 8\%\end{tabular} \\
CLIP-RN50x64/14 &  \begin{tabular}[c]{@{}l@{}}7\% 23\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}0\% 11\%\end{tabular} \\
LiT             &  \begin{tabular}[c]{@{}l@{}}\textbf{48\%} \textbf{50\%}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{23\%} \textbf{26\%}\end{tabular} \\ \bottomrule

\end{tabular}}
\caption{Zero-shot models performance on the idioms understanding task with partially literal distractors. Numbers are the percentage of instances annotated correctly. There are two configurations with 2 and 4 candidates. The table is double-columned. The left column shows the score for the phrase alone as input, and the right column shows the score for the phrase and its definitions as input.}
\label{tab:partial-objects-idiom-single-choice-results}
\end{table}





